An Efficient Framework for Global Non-Convex Polynomial Optimization with Algebraic Constraints

We present an efficient framework for solving algebraically-constrained global non-convex polynomial optimization problems over subsets of the hypercube. We prove the existence of an equivalent nonlinear reformulation of such problems that possesses essentially no spurious local minima. Through numerical experiments on previously intractable global constrained polynomial optimization problems in high dimension, we show that polynomial scaling in dimension and degree is achievable when computing the optimal value and location.

==> bkup.tex <==
\subsection{Observations and technical details}

This sections discusses some of our observations using the numerical solver. 

First, it is worth mentioning that, for most of of our experiments, \texttt{Ipopt} was able to reach its termination criteria and reported a successful solve status. Occasionally, however, \texttt{Ipopt} would fail to terminate appropriately. We observed one main specific cause for this behavior: an error in a step computation. We succeeded in resolving the step computation error by turning off the first order approximation or when restarting with a different random initialization.


Secondly, we also observed issues with the automatic differentiation of the \texttt{Forwarddiff.jl} package when used in conjunction the \texttt{DynamicPolynomials.jl} package \cite{benoit_legat_2023_8329719} for expressing polynomials.

so we parsed these polynomials into our own, stripped-down polynomial data structures. We suspect that more efficiently computing gradients by hand will provide substantial speedups, and so this optimization is the subject of future work. 
